Model Accuracy and Runtime Tradeoff in Distributed Deep Learning:A Systematic Study

This paper presents Rudra, a parameter server based distributed computing framework tuned for training large-scale deep neural networks. Using variants of the asynchronous stochastic gradient descent algorithm we study the impact of synchronization protocol, stale gradient updates, minibatch size, learning rates, and number of learners on runtime performance and model accuracy. We introduce a new learning rate modulation strategy to counter the effect of stale gradients and propose a new synchronization protocol that can effectively bound the staleness in gradients, improve runtime performance and achieve good model accuracy. Our empirical investigation reveals a principled approach for distributed training of neural networks: the mini-batch size per learner should be reduced as more learners are added to the system to preserve the model accuracy. We validate this approach using commonly-used image classification benchmarks: CIFAR10 and ImageNet.

==> Makefile <==
.SUFFIXES: .eps .pdf
LATEX=./colourlatex.sh pdflatex
BIBTEX=bibtex
FIG2DEV=fig2dev

NAME=main
#BIBNAME=acmsmall-sample-bibfile
BIBNAME=sigproc

all: $(NAME).pdf $(NAME).ps

#FIGSEPS=$(shell ls -1 figs/*.eps)

#RESULTSEPS=$(shell ls -1 results/*.eps)

#EPS=$(FIGSEPS) $(RESULTSEPS)
TEX=$(NAME).tex \
    $(BIBNAME).bib \

$(NAME).dvi: $(TEX) $(EPS) $(BIBNAME).bbl
	@echo Compiling $(NAME)
	@$(LATEX) $(NAME)
	@$(MAKE) fixlabels

$(NAME).pdf: $(NAME).dvi
	@dvipdfmx -p letter $(NAME).dvi

$(NAME).ps: $(NAME).dvi
	@dvips $(NAME).dvi
	@pkill -HUP -f "^gv .*$@" || true


fixlabels:
ifneq ($(shell grep -s -c 'Label(s) may have changed. Rerun to get cross-references right.' $(NAME).log),0)
	@echo $(NAME) Compiling again to fix labels
	@$(LATEX) $(NAME)
else
	@echo $(NAME) Labels are correct
endif

$(BIBNAME).bbl: $(BIBNAME).bib
	@echo Compiling required EPS files
	#@make -C figs
	@echo Compiling main for bibliography
	@$(LATEX) $(NAME)
	@echo Generating bibliography
	@$(BIBTEX) $(NAME)
	@echo Recompiling main after generating bibliography
	@$(LATEX)  $(NAME)
	@$(MAKE) fixlabels

%.eps.pdf: %.eps
	@echo "	" Converting $< to $(@)
	@epstopdf --outfile=figs/$(@) $<

clean:
	#@make -C figs clean
	@/bin/rm -f $(NAME).ps $(NAME).pdf *.aux *.dvi *.log *.bbl *.blg figs/*.pdf *.toc *.out *.bak


==> Makefile_tmp <==
.SUFFIXES: .eps .pdf
LATEX=./colourlatex.sh pdflatex
BIBTEX=bibtex
FIG2DEV=fig2dev

NAME=main
#BIBNAME=acmsmall-sample-bibfile
BIBNAME=sigproc

all: $(NAME).pdf $(NAME).ps

#FIGSEPS=$(shell ls -1 figs/*.eps)

#RESULTSEPS=$(shell ls -1 results/*.eps)

#EPS=$(FIGSEPS) $(RESULTSEPS)
TEX=$(NAME).tex \
    $(BIBNAME).bib \

$(NAME).dvi: $(TEX) $(EPS) $(BIBNAME).bbl
	@echo Compiling $(NAME)
	@$(LATEX) $(NAME)
	@$(MAKE) fixlabels

$(NAME).pdf: $(NAME).dvi
	@dvipdfmx -p letter $(NAME).dvi

$(NAME).ps: $(NAME).dvi
	@dvips $(NAME).dvi
	@pkill -HUP -f "^gv .*$@" || true


fixlabels:
ifneq ($(shell grep -s -c 'Label(s) may have changed. Rerun to get cross-references right.' $(NAME).log),0)
	@echo $(NAME) Compiling again to fix labels
	@$(LATEX) $(NAME)
else
	@echo $(NAME) Labels are correct
endif

$(BIBNAME).bbl: $(BIBNAME).bib
	@echo Compiling required EPS files
	#@make -C figs
	@echo Compiling main for bibliography
	@$(LATEX) $(NAME)
	@echo Generating bibliography
	@$(BIBTEX) $(NAME)
	@echo Recompiling main after generating bibliography
	@$(LATEX)  $(NAME)
	@$(MAKE) fixlabels

%.eps.pdf: %.eps
	@echo "	" Converting $< to $(@)
	@epstopdf --outfile=figs/$(@) $<

clean:
	#@make -C figs clean
	@/bin/rm -f $(NAME).ps $(NAME).pdf *.aux *.dvi *.log *.bbl *.blg figs/*.pdf *.toc *.out *.bak


==> idea.tex <==
(1) we are getting table AMAZING, under the assumption that EPOCH number is fixed. In a traditional HPC problem, when EPOCH number is fixed, that means the same workload is fixed. In a new workload like DNN, given fixed amount of workload, the model quality can be very much different. If the goal is to hit the accuracy dictated by the \lambda*\mu, then one can expect to see a linear speedup. 

However, one should never expect to see linear speedup to hit the accuracy, if the accuracy is set to be high  

